The Value Equivalence Principle for Model-Based Reinforcement Learning

Learning models of the environment from data is often viewed as an essential component to building intelligent reinforcement learning (RL) agents. The common practice is to separate the learning of the model from its use, by constructing a model of the environment's dynamics that correctly predicts the observed state transitions. In this paper we argue that the limited representational resources of model-based RL agents are better used to build models that are directly useful for value-based planning. As our main contribution, we introduce the principle of value equivalence: two models are value equivalent with respect to a set of functions and policies if they yield the same Bellman updates. We propose a formulation of the model learning problem based on the value equivalence principle and analyze how the set of feasible solutions is impacted by the choice of policies and functions. Specifically, we show that, as we augment the set of policies and functions considered, the class of value equivalent models shrinks, until eventually collapsing to a single point corresponding to a model that perfectly describes the environment. In many problems, directly modelling state-to-state transitions may be both difficult and unnecessary. By leveraging the value-equivalence principle one may find simpler models without compromising performance, saving computation and memory. We illustrate the benefits of value-equivalent model learning with experiments comparing it against more traditional counterparts like maximum likelihood estimation. More generally, we argue that the principle of value equivalence underlies a number of recent empirical successes in RL, such as Value Iteration Networks, the Predictron, Value Prediction Networks, TreeQN, and MuZero, and provides a first theoretical underpinning of those results.

==> excerpts.tex <==

% \begin{restatable}{proposition}{propvip}
% Consider the MRP induced by policy $\pi$ shown in Figure~\ref{fig:example_mrp}. Let $\VV = [[1, 0, 0]^\t, [0, 1, 1]^\t]$. Then, for any instantitation of the rewards $r, r_1, r_2,$ and $r_3$, any transition matrix $\P \in \PP(\{\pi\}, \VV) \subset \R^{3 \times 3}$ will yield an exact value function $\vt_{\pi} = v_{\pi}$.
% \label{thm:vip}
% \end{restatable}

Based on Proposition~\ref{thm:vip}, it is easy to construct an example of a model class $\PP' \subset \PP$ such that the value equivalence loss~(\ref{eq:ve_loss}) leads to an exact value function $\vt_{\pi} = v_{\pi}$ while the MLE loss~(\ref{eq:cml_p}) does not. To simplify, suppose we have $\pt_{21} = \pt_{31} = 1$ and we are only interested in approximating the transition probabilities $p_{11}, p_{12}$, and $p_{13}$ ({\sl cf.}~Figure~\ref{fig:example_mrp}). We use a single parameter $\theta \in \R$ to represent $\pt_{11}, \pt_{12}$, and $\pt_{13}$, in the following way: 
\begin{equation*}
\label{eq:rep_p2}
\pt_{12} = \theta \text{ and } \pt_{11} = \pt_{13} = (1-\theta)/2, \text{ with } \theta \in [0,1].
\end{equation*}
Clearly, by making $\theta = 1 - 2p_{13}$, we have a model $\Pt \in \PP(\{\pi\}, \VV)$---which means that minimization of~(\ref{eq:ve_loss}) yields an exact model. However, it is easy to verify that the MLE solution resuting from the minimization of~(\ref{eq:cml_p}) will result in $\theta = p_{12}$ (see proof of Proposition~\ref{thm:mle} in Appendix~\ref{sec:proofs}). This means that the solution found by MLE will be inexact whenever $p_{12} \ne p_{13}$.


Proposition~\ref{thm:vip} elucidates a condition under which $\vec{\V}_v \subseteq \V'$. Because \Tpi\ are contraction mappings, given a function $v$, it is always possible to define a $\V'$ such that the condition holds: if we define balls around the operators' fixed points that are big enough to include $v$, the union of such balls will be a valid $\V'$. But in some cases it is possible to define a less trivial $\V'$. In Appendix~\ref{sec:proofs} we give an example of a finite state-space MDP in which it is possible to define a $\V'$ such that $\dim(\V') = k < |S|$ (that is, the operators \Tpi\ will map a subspace of $\R^{|S|}$ onto itself). Building on this example, it is easy to define a class $\M$ such that the value equivalence loss~(\ref{eq:ve_loss}) leads to the optimal solution while the MLE loss~(\ref{eq:cml_p}) does not, which illustrates Proposition~\ref{thm:mle} (see App.~\ref{sec:proofs}). Although in general we do not have access to $\V'$, in some cases this set will be revealed through the very process of enforcing value equivalence. For example, suppose \mt\ is being learned online based on a sequence of functions $v_1, v_2 = \Tpi v_1, v_3 = \T_{\pi'} v_2, ...$. Since once the sequence reaches a $v_i \in \V'$ it stays there forever, we should expect the model to eventually specialize to $\V'$~\cp{farahmand2018iterative}.


==> experiments_bk.tex <==
In the previous section we outlined two potential strategies to select \V: \textbf{(1)} using actual value functions associated with arbitrary policies, and
\textbf{(2)} using a basis of the class of functions the agent uses to
represent value functions. We will refer to these as \emph{value function} and \emph{basis} strategies, respectively. In what follows will present experiments illustrating the benefits of value-equivalence model training using each.
For all experiments we used $\Pi = \{ \pi^a \}_{a \in \A}$ where $\pi^a(a | s) = 1$ for all $s \in \S$, so we restrict our focus to \V. 

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{./fig/tabular_environments.pdf}
\caption{Illustration of tabular domains used in experiments. \textbf{(a)} Four Room domain: an agent (orange square) can move up, down, left and right. The agent is blocked by walls (grey). There is a single rewarding square (green) in the top left corner that the agent recieves a reward of $1$ for transitioning into. \textbf{(b)} Catch domain: an agent controls a paddle (orange) which it can move left, right or choose to stay in place. A ball (blue) descends directly downward from a randomly selected square at the top of the grid. If the agent's paddle occupies the same column as the ball when it reaches the bottom of the grid, the agent receives a reward of $1$. }
\label{fig:tabular_envs}
\end{figure}

\subsection{Environments}
We illustrate the benefits of value equivalence across three common RL environments: Four Rooms, Catch and Cartpole.
These environments are depicted in Figure \ref{fig:tabular_envs}. 
Four Rooms and Catch are both tabular environments that allow for us showcase the benefits of value equivalent models in a pure setting without introducing function approximation for our models.
We include Cartpole with its continuous state-space to illustrate that our results carry over to the more realistic setting where nonlinear function approximation is used for both the model and value function approximation.

\subsection{Shared experimental procedure} 
Unless stated otherwise, our experiments follow a common procedure:
\begin{enumerate}
\item \textbf{Data Collection}: Collect experience tuples $\{(s_i, a_i, r_i, s^\prime_i)\}_{i=1}^N$ are collected with a uniform random policy
\item \textbf{Model Training}: A model is trained using MLE to minimise Eqs. (\ref{eq:cml_r}, \ref{eq:cml_p}) or VE to minimise Eq. (\ref{eq:ve_loss_emp}).
\item \textbf{Policy Construction}: An optimal policy with respect to the model is computed. 
\item \textbf{Policy Evaluation}: The policy is evaluated on the true environment. 
\end{enumerate}

\subsection{Tabular basis strategy  experiments} \ref{sec:tabular_basis_strategy}
First we consider the setting where a tabular model is learned and used with a linear value function approximator. 
We investigate the interaction between the capacities of the model and the value function approximator by restricting each.
We show empirically that models learned to be value equivalent model to a basis of the value function-approximator's function class are more robust than those learned with maximum likelihood estimation.

The model, $\{ \boldsymbol{\tilde{P}}^a \}_{a \in \mathcal{A}}$, is ``rank restricted,'' meaning that each matrix $\rank(\boldsymbol{\tilde{P}}^a) \leq k$ for some $k$. 
This is enforced by representing each $\boldsymbol{\tilde{P}}^a$ as the matrix product: $\boldsymbol{D}^a \boldsymbol{K}^a$ where $\boldsymbol{D}^a \in \mathbb{R}^{|S| \times k}$, $\boldsymbol{K}^a \in \mathbb{R}^{k \times |S|}$ and both are row-stochastic matrices.

The value function approximator is restricted through its function class. 
We achieve this by constructing state aggregations and requiring that all states in the same aggregated state have the same value.
This is equivalent to requiring that $\mathcal{V} = \{ \tilde{v}_w | \tilde{v}_w(s) = \sum_{i=1}^d w_i \boldsymbol{1}_{s \in C_i} \}$ where $w \in \mathbb{R}^d$ and $C_{1:d}$ are aggregated states clusters.
For these experiments we set $\boldsymbol{V} = \{f_i(s) = \boldsymbol{1}_{s \in C_i}\}_{i=1}^d$.
We construct clusters by first using a random uniform policy to collect samples of states then applying k-means clustering on the sampled states and associating each state with its closest centroid. 



\textbf{Model Training:} 
All models are trained using gradient descent with the Adam optimizer and a learning rate of $5\text{e-}5$. 
Matrices are constrained to be row-stochastic by representing them as $P = \text{softmax}(F)$ where $F \in \mathbb{R}^{n \times n}$ and $\text{softmax}(\cdot)$ is a row-wise softmax operator. 

To train our rank-restricted models in the tabular setting we first construct an unrestricted estimate of the dynamics:
$\bar{P}^a_{s,s^\prime} = (\sum_{i=1}^N \boldsymbol{1}_{s_i=s \wedge s^\prime_i=s^\prime}) / N$, $\bar{R}^a_{s} =  (\sum_{i=1}^N r_i) / N$.
For MLE models we then optimise  $\min_{\boldsymbol{\tilde{P}}} \sum_{a \in \mathcal{A}} D_{KL}(\boldsymbol{\tilde{P}}^a || \bar{P}^a)$.
For VE models we optimise $\min_{\boldsymbol{\tilde{P}}} \sum_{a \in \mathcal{A}} \|  \boldsymbol{\tilde{P}}^a \boldsymbol{V} - \bar{P}^a \boldsymbol{V} \|_F^2$.

\textbf{Policy Construction:} 
We produce a policy by performing policy iteration with least squares temporal-difference learning (LSTD) for our policy evaluation step.
LSTD evaluates a policy by collecting on-policy experience tuples $(s, a, r, s')$ acting according to it. 
We make use of our model by replacing $r$ and $s$ in each of these tuples with the model's predicted next state and reward.
After each policy evaluation, we use the resulting value estimate: $v_w(s)$ along with our model to produce an improved policy: $\pi'(s) = \text{argmax}_a \bar{R}_a + \gamma \mathbb{E}_{s' \sim \boldsymbol{\tilde{P}}^a}[v_w(s')]$.
We perform $20$ iterations of policy iteration in this manner and evaluate the final policy.

\textbf{Policy Evaluation:}
Once a policy $\pi$ has been produced we compute its exact value with respect to the true environment: $v^\pi$. We then report $(1/|S|) \sum_{s \in \mathcal{S}} v^\pi(s)$ as a summary of the model's quality. 

The results of this experiment are reported in Figure \ref{fig:full_basis_tabular}. 
\begin{figure}
\centering
\includegraphics[width=\textwidth]{./fig/full_basis_tabular}
\caption{Tabular Basis Strategy Experiment}
\label{fig:full_basis_tabular}
\end{figure}


\subsection{Tabular policy strategy experiments}
Next we empirically illustrate the policy strategy where, rather than using the basis of the agent's value function approximator's function space, we use actual value functions associated with randomly sampled deterministic policies. 

For this experiment we randomly sample a fixed number of deterministic policies $\{\pi_i\}_{i=1}^d$ and evaluate them to produce $\{v^{\pi_i}\}_{i=1}^d$.
We set $\boldsymbol{V} = \{v^{\pi_i}\}_{i=1}^d$. 

The experimental setup has the same Data Collection, Model Training and Policy Evaluation phases as in the previous subsection.

\textbf{Policy Construction}:
Since this experiment is not concerned with restrictions on the space of value functions that the agent can represent, we do not need to use LSTD for policy evaluation.
Instead we simply apply tabular Q-iteration using the learned model in place of the environment to directly produce a policy.

The results of this experiment are displayed in Figure~\ref{fig:pi_basis_tabular}.


\begin{figure}
\centering
\includegraphics[width=\textwidth]{./fig/pi_basis_tabular}
\caption{Tabular Policy Strategy Experiment}
\label{fig:pi_basis_tabular}
\end{figure}

\subsection{Nontabular basis strategy experiments}
Up until now we've only consider experiments on tabular domains. 
We now repeat the Basis Strategy experiment using Cartpole with nonlinear function approximation for both the model and the agent's value function approximator. 
We focus specifically on the effect of restricting the model's capacity while keeping the value function approximator's function class fixed as the set of learnable neural networks with 2 hidden layers with 256 units each and tanh activations. 

In what follows we will list the manner differences between Subsection \ref{sec:tabular_basis_strategy}.

\textbf{Data Collection:}
Unlike previous domains Cartpole requires some degree of exploration to achieve good policies.
Since this is not the focus of our work, we modify the initial-state distribution to include the full spectrum of cart position.

\textbf{Model Training:}
Instead of using a set of matrices as our model, the continuous state-space of Cartpole requires us to use an expectation model: $f_\theta(s, a) = $

\begin{itemize}
\item We now illustrate how to use VE in practice.
\item Show experiments in this order:
\begin{itemize}
\item Finite \S\ and linear function approximation.
\begin{itemize}
\item  Here the model $m$ is a matrix $\Pt = \DD \KK$.
\end{itemize}
\item Continuous \S\ and linear function approximation.
\begin{itemize}
\item  Here we use an expectation model $\ft(s,a) = \E_{S' \sim p(\cdot | s,a)}[S']$.
\item  Note that, because \vt\ is linear, we can write $\E_{S' \sim p}[\vt(S')] = \vt(\E_{S' \sim p}[S'])$.
\item  To control the complexity of $\ft$ we regularize the neural network.
\end{itemize}
\item Continuous \S\ and non-linear function approximation.
\begin{itemize}
\item  Here we again use an expectation model $\ft(s,a) = \E_{S' \sim p(\cdot | s,a)}[S']$.
\item  In order to use a non-linear function approximation \vt, the environment must have deterministic dynamics.
\item  As before, to control the complexity of $\ft$ we regularize the neural network.
\end{itemize}
\end{itemize}
\end{itemize}


==> motivation.tex <==
Given a state space \S\ and an action space \A, we call the tuple $m \defi (r,p)$ a \emph{model}. Note that a model plus a discount factor $\gamma$ induces a Bellman operator~(\ref{eq:bo}) for every policy $\pi \in \PS$. In this paper we are interested in computing an approximate model $\mt = (\rt, \pt)$ such that the induced operators $\Tpit$, defined analogously to~(\ref{eq:bo}), are good approximations of the true $\Tpi$. 

% \begin{wrapfigure}{r}{0.35\textwidth}
% \begin{center}
% \includegraphics[scale=0.75]{./fig/example_mrp}
% \end{center}
% \caption{ MRP induced by $\pi$. \label{fig:example_mrp} } 
% \vspace{-5mm}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.5\textwidth}
\begin{center}
\subfigure[MRP\label{fig:example_mrp_split}]{
\includegraphics[scale=0.75]{./fig/example_mrp_split}
}
\subfigure[Alternate MRP \label{fig:example_mrp_one}]{
\includegraphics[scale=0.75]{./fig/example_mrp_one}
}
\end{center}
\caption{Example of equivalent models}
\label{fig:example_mrp}
\vspace{-5mm}
\end{wrapfigure}

We start with a motivating example. Suppose we are interested in evaluating policy $\pi$ whose behavior is described by the Markov reward process (MRP) shown in Figure~\ref{fig:example_mrp_split} (that is, $\pi$ induces on an MDP the transition probabilities and rewards shown). 
In the figure, the pairs over each arrow indicate the probability of transitioning along it and the reward obtained for doing so.
We want to compute approximations $\pt \approx p$ and $\rt \approx r$ and use them to estimate the  policy's value function, $\vt_{\pi} \approx v_{\pi}$. 

Clearly, if $\rt = r$ and $\pt = p$, we have that $\vt_{\pi} = v_{\pi}$. 
But this is not the only solution that yields an exact value function. 
Observe that while in $s_1$ the agent will uniformly transition to either $s_2$ or $s_3$, receiving no reward. 
Thereafter the agent necessarily transitions to $s_1$ and receives a reward of $10$. 
This equivalence of outcome indicates that the proportion with which $s_1$ transitions to $s_2$ or $s_3$ does not affect the value of the MRP. 
Indeed, we can construct an alternate MRP that yields the same evaluation of $\pi$, as depicted in Figure~\ref{fig:example_mrp_one}. 
This suggests there is a \emph{space of models} that lead to the correct evaluation of $\pi$. Although these models are indistinguishable with respect to the computation of $\vt_{\pi}$, some of them can be easier to learn and use than others, much like the alternate MRP in Figure~\ref{fig:example_mrp_one} largely disregards $s_3$. In this paper we show that this and other model spaces of interest can be expressed as an equivalence relation induced by a set of policies and functions. 


% Observe that, while following policy $\pi$, whenever the agent is in states $s_2$ or $s_3$ it deterministically transitions to state $s_1$ and gets a reward of $r$.  This means that, in order for a model to be accurate, it only needs to capture the \emph{expected effect} associated with transitioning to $s_2$ and $s_3$. To be more precise, suppose that $\rt_1 = r_1$, $\rt = r$, $\pt_{11} = p_{11}$ and $\pt_{31} = \pt_{21} = 1$. Then, it is easy to verify that, as long as $\pt_{12} \rt_2 + \pt_{13} \rt_3 = p_{12} r_2 + p_{13} r_3$, the resulting $\vt_{\pi}$ is exact. This defines a \emph{space of models} that lead to the correct evaluation of $\pi$. Although these models are indistinguishable with respect to the computation of $\vt_{\pi}$, some of them can be easier to learn and use than others. For example, one possible solution for our example is to have $\rt_2 = p_{12} r_2 + p_{13} r_3$, $\pt_{12} = p_{12} + p_{13}$ and  $\pt_{13} = 0$, which allows us to exclude $s_3$ from the iterative process defined in~(\ref{eq:bo}). In this paper we show that this and other model spaces of interest can be expressed as an equivalence relation induced by a set of policies and functions. 
     

==> refs.tex <==
\begin{thebibliography}{21}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Barto et~al.(1983)Barto, Sutton, and Anderson]{barto1983neuronlike}
Andrew~G Barto, Richard~S Sutton, and Charles~W Anderson.
\newblock Neuronlike adaptive elements that can solve difficult learning
  control problems.
\newblock \emph{IEEE transactions on systems, man, and cybernetics}, \penalty0
  (5):\penalty0 834--846, 1983.

\bibitem[Bellemare et~al.(2019)Bellemare, Dabney, Dadashi, Taiga, Castro,
  Le~Roux, Schuurmans, Lattimore, and Lyle]{bellemare2019geometric}
Marc Bellemare, Will Dabney, Robert Dadashi, Adrien~Ali Taiga, Pablo~Samuel
  Castro, Nicolas Le~Roux, Dale Schuurmans, Tor Lattimore, and Clare Lyle.
\newblock A geometric perspective on optimal representations for reinforcement
  learning.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  4360--4371, 2019.

\bibitem[Bertsekas and Tsitsiklis(1996)]{bertsekas96neuro-dynamic}
Dimitri~P. Bertsekas and John~N. Tsitsiklis.
\newblock \emph{Neuro-Dynamic Programming}.
\newblock Athena Scientific, 1996.

\bibitem[Dadashi et~al.(2019)Dadashi, Taiga, Roux, Schuurmans, and
  Bellemare]{dadashi2019value}
Robert Dadashi, Adrien~Ali Taiga, Nicolas~Le Roux, Dale Schuurmans, and Marc~G.
  Bellemare.
\newblock The value function polytope in reinforcement learning.
\newblock In \emph{Proceedings of the International Conference on Machine
  Learning ({ICML})}, volume~97, pages 1486--1495, 2019.

\bibitem[Farahmand(2018)]{farahmand2018iterative}
Amir{-}massoud Farahmand.
\newblock Iterative value-aware model learning.
\newblock In \emph{Advances in Neural Information Processing Systems
  ({NeurIPS})}, pages 9090--9101, 2018.

\bibitem[Farahmand et~al.(2017)Farahmand, Barreto, and
  Nikovski]{farahmand2017value}
Amir-Massoud Farahmand, Andr\'{e} Barreto, and Daniel Nikovski.
\newblock {Value-Aware Loss Function for Model-based Reinforcement Learning}.
\newblock In \emph{Proceedings of the International Conference on Artificial
  Intelligence and Statistics ({AISTATS})}, volume~54, pages 1486--1494, 2017.

\bibitem[Farquhar et~al.(2018)Farquhar, Rockt{\"a}schel, Igl, and
  Whiteson]{farquhar2018treeqn}
G~Farquhar, T~Rockt{\"a}schel, M~Igl, and S~Whiteson.
\newblock Treeqn and atreec: Differentiable tree-structured models for deep
  reinforcement learning.
\newblock In \emph{6th International Conference on Learning Representations,
  ICLR 2018-Conference Track Proceedings}, volume~6. ICLR, 2018.

\bibitem[Joseph et~al.(2013)Joseph, Geramifard, Roberts, How, and
  Roy]{joseph2013reinforcement}
Joshua Joseph, Alborz Geramifard, John~W Roberts, Jonathan~P How, and Nicholas
  Roy.
\newblock Reinforcement learning with misspecified model classes.
\newblock In \emph{2013 IEEE International Conference on Robotics and
  Automation}, pages 939--946. IEEE, 2013.

\bibitem[Millar(2011)]{milar2003maximum}
Russell~B. Millar.
\newblock \emph{Maximum Likelihood Estimation and Inference}.
\newblock Hoboken: Wiley, 2011.

\bibitem[Mnih et~al.(2014)Mnih, Heess, Graves, and
  Kavukcuoglu]{mnih2014recurrent}
Volodymyr Mnih, Nicolas Heess, Alex Graves, and Koray Kavukcuoglu.
\newblock Recurrent models of visual attention.
\newblock In \emph{Advances in neural information processing systems ({NIPS})},
  pages 2204--2212, 2014.

\bibitem[Oh et~al.(2017)Oh, Singh, and Lee]{oh2017value}
Junhyuk Oh, Satinder Singh, and Honglak Lee.
\newblock Value prediction network.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  6118--6128, 2017.

\bibitem[Puterman(1994)]{puterman94markov}
Martin~L. Puterman.
\newblock \emph{Markov Decision Processes---Discrete Stochastic Dynamic
  Programming}.
\newblock John Wiley \& Sons, Inc., 1994.

\bibitem[Russell and Norvig(2003)]{russel2003artificial}
Stuart~J. Russell and Peter Norvig.
\newblock \emph{Artificial Intelligence: A Modern Approach}.
\newblock Pearson Education, 3 edition, 2003.

\bibitem[Schrittwieser et~al.(2019)Schrittwieser, Antonoglou, Hubert, Simonyan,
  Sifre, Schmitt, Guez, Lockhart, Hassabis, Graepel,
  et~al.]{schrittwieser2019mastering}
Julian Schrittwieser, Ioannis Antonoglou, Thomas Hubert, Karen Simonyan,
  Laurent Sifre, Simon Schmitt, Arthur Guez, Edward Lockhart, Demis Hassabis,
  Thore Graepel, et~al.
\newblock Mastering atari, go, chess and shogi by planning with a learned
  model.
\newblock \emph{arXiv preprint arXiv:1911.08265}, 2019.

\bibitem[Silver et~al.(2017)Silver, van Hasselt, Hessel, Schaul, Guez, Harley,
  Dulac-Arnold, Reichert, Rabinowitz, Barreto, et~al.]{silver2017predictron}
David Silver, Hado van Hasselt, Matteo Hessel, Tom Schaul, Arthur Guez, Tim
  Harley, Gabriel Dulac-Arnold, David Reichert, Neil Rabinowitz, Andre Barreto,
  et~al.
\newblock The predictron: End-to-end learning and planning.
\newblock In \emph{Proceedings of the 34th International Conference on Machine
  Learning-Volume 70}, pages 3191--3199. JMLR. org, 2017.

\bibitem[Sutton(1988)]{sutton88learning}
Richard~S. Sutton.
\newblock Learning to predict by the methods of temporal differences.
\newblock \emph{Machine Learning}, 3:\penalty0 9--44, 1988.

\bibitem[Sutton and Barto(2018)]{sutton2018reinforcement}
Richard~S. Sutton and Andrew~G. Barto.
\newblock \emph{Reinforcement Learning: An Introduction}.
\newblock MIT Press, 2018.
\newblock URL
  \url{https://mitpress.mit.edu/books/reinforcement-learning-second-edition}.
\newblock 2nd edition.

\bibitem[Sutton et~al.(1999)Sutton, Precup, and Singh]{sutton1999between}
Richard~S Sutton, Doina Precup, and Satinder Singh.
\newblock Between mdps and semi-mdps: A framework for temporal abstraction in
  reinforcement learning.
\newblock \emph{Artificial intelligence}, 112\penalty0 (1-2):\penalty0
  181--211, 1999.

\bibitem[Sutton et~al.(2008)Sutton, Szepesv\'{a}ri, Geramifard, and
  Bowling]{sutton2008dyna}
Richard~S. Sutton, Csaba Szepesv\'{a}ri, Alborz Geramifard, and Michael
  Bowling.
\newblock Dyna-style planning with linear function approximation and
  prioritized sweeping.
\newblock In \emph{Proceedings of the Conference on Uncertainty in Artificial
  Intelligence ({UAI})}, page 528–536, 2008.

\bibitem[Szepesv{\'a}ri(2010)]{szepesvari2010algorithms}
Csaba Szepesv{\'a}ri.
\newblock \emph{Algorithms for Reinforcement Learning}.
\newblock Synthesis Lectures on Artificial Intelligence and Machine Learning.
  Morgan {\&} Claypool Publishers, 2010.

\bibitem[Tamar et~al.(2016)Tamar, Wu, Thomas, Levine, and
  Abbeel]{tamar2016value}
Aviv Tamar, Yi~Wu, Garrett Thomas, Sergey Levine, and Pieter Abbeel.
\newblock Value iteration networks.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  2154--2162, 2016.

\end{thebibliography}


==> refs2.tex <==
\begin{thebibliography}{29}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Asadi et~al.(2018)Asadi, Cater, Misra, and
  Littman]{asadi2018equivalence}
Kavosh Asadi, Evan Cater, Dipendra Misra, and Michael~L. Littman.
\newblock Equivalence between wasserstein and value-aware model-based
  reinforcement learning.
\newblock In \emph{{FAIM} Workshop on Prediction and Generative Modeling in
  Reinforcement Learning}, 2018.
% 
% \bibitem[Barto et~al.(1983)Barto, Sutton, and Anderson]{barto1983neuronlike}
% Andrew~G Barto, Richard~S Sutton, and Charles~W Anderson.
% \newblock Neuronlike adaptive elements that can solve difficult learning
%   control problems.
% \newblock \emph{IEEE transactions on systems, man, and cybernetics}, \penalty0
%   (5):\penalty0 834--846, 1983.
% 
% \bibitem[Bellemare et~al.(2019)Bellemare, Dabney, Dadashi, Taiga, Castro,
%   Le~Roux, Schuurmans, Lattimore, and Lyle]{bellemare2019geometric}
% Marc Bellemare, Will Dabney, Robert Dadashi, Adrien~Ali Taiga, Pablo~Samuel
%   Castro, Nicolas Le~Roux, Dale Schuurmans, Tor Lattimore, and Clare Lyle.
% \newblock A geometric perspective on optimal representations for reinforcement
%   learning.
% \newblock In \emph{Advances in Neural Information Processing Systems}, pages
%   4360--4371, 2019.
% 
% \bibitem[Bertsekas and Tsitsiklis(1996)]{bertsekas96neuro-dynamic}
% Dimitri~P. Bertsekas and John~N. Tsitsiklis.
% \newblock \emph{Neuro-Dynamic Programming}.
% \newblock Athena Scientific, 1996.
% 
% \bibitem[Dadashi et~al.(2019)Dadashi, Taiga, Roux, Schuurmans, and
%   Bellemare]{dadashi2019value}
% Robert Dadashi, Adrien~Ali Taiga, Nicolas~Le Roux, Dale Schuurmans, and Marc~G.
%   Bellemare.
% \newblock The value function polytope in reinforcement learning.
% \newblock In \emph{Proceedings of the International Conference on Machine
%   Learning ({ICML})}, volume~97, pages 1486--1495, 2019.
% 
% \bibitem[Farahmand(2018)]{farahmand2018iterative}
% Amir{-}massoud Farahmand.
% \newblock Iterative value-aware model learning.
% \newblock In \emph{Advances in Neural Information Processing Systems
%   ({NeurIPS})}, pages 9090--9101, 2018.
% 
\bibitem[Farahmand et~al.(2013)Farahmand, Barreto, and
  Nikovski]{farahmand2013value}
Amir-Massoud Farahmand, Andr\'{e} Barreto, and Daniel Nikovski.
\newblock {Value-aware loss function for model learning in reinforcement
  learning}.
\newblock In \emph{Proceedings of the European Workshop on Reinforcement
  Learning ({EWRL})}, 2013.
% 
% \bibitem[Farahmand et~al.(2017)Farahmand, Barreto, and
%   Nikovski]{farahmand2017value}
% Amir-Massoud Farahmand, Andr\'{e} Barreto, and Daniel Nikovski.
% \newblock {Value-Aware Loss Function for Model-based Reinforcement Learning}.
% \newblock In \emph{Proceedings of the International Conference on Artificial
%   Intelligence and Statistics ({AISTATS})}, volume~54, pages 1486--1494, 2017.
% 
% \bibitem[Farquhar et~al.(2018)Farquhar, Rockt{\"a}schel, Igl, and
%   Whiteson]{farquhar2018treeqn}
% G~Farquhar, T~Rockt{\"a}schel, M~Igl, and S~Whiteson.
% \newblock Treeqn and atreec: Differentiable tree-structured models for deep
%   reinforcement learning.
% \newblock In \emph{6th International Conference on Learning Representations,
%   ICLR 2018-Conference Track Proceedings}, volume~6. ICLR, 2018.
% 
\bibitem[Ferns et~al.(2004)Ferns, Panangaden, and Precup]{ferns2004metrics}
Norman Ferns, Prakash Panangaden, and Doina Precup.
\newblock Metrics for finite markov decision processes.
\newblock In \emph{UAI}, 2004.
% 
% \bibitem[Joseph et~al.(2013)Joseph, Geramifard, Roberts, How, and
%   Roy]{joseph2013reinforcement}
% Joshua Joseph, Alborz Geramifard, John~W Roberts, Jonathan~P How, and Nicholas
%   Roy.
% \newblock Reinforcement learning with misspecified model classes.
% \newblock In \emph{2013 IEEE International Conference on Robotics and
%   Automation}, pages 939--946. IEEE, 2013.
% 
\bibitem[Li et~al.(2006)Li, Walsh, and Littman]{li2006towards}
Lihong Li, Thomas~J. Walsh, and Michael~L. Littman.
\newblock Towards a unified theory of state abstraction for {MDPs}.
\newblock In \emph{Proceedings of the International Symposium on Artificial
  Intelligence and Mathematics}, pages 531--539, 2006.
% 
% \bibitem[Millar(2011)]{milar2003maximum}
% Russell~B. Millar.
% \newblock \emph{Maximum Likelihood Estimation and Inference}.
% \newblock Hoboken: Wiley, 2011.
% 
% \bibitem[Mnih et~al.(2014)Mnih, Heess, Graves, and
%   Kavukcuoglu]{mnih2014recurrent}
% Volodymyr Mnih, Nicolas Heess, Alex Graves, and Koray Kavukcuoglu.
% \newblock Recurrent models of visual attention.
% \newblock In \emph{Advances in neural information processing systems ({NIPS})},
%   pages 2204--2212, 2014.
% 
% \bibitem[Oh et~al.(2017)Oh, Singh, and Lee]{oh2017value}
% Junhyuk Oh, Satinder Singh, and Honglak Lee.
% \newblock Value prediction network.
% \newblock In \emph{Advances in Neural Information Processing Systems}, pages
%   6118--6128, 2017.
% 
\bibitem[Poupart and Boutilier(2002)]{poupart2002value}
Pascal Poupart and Craig Boutilier.
\newblock Value-directed compression of pomdps.
\newblock In Suzanna Becker, Sebastian Thrun, and Klaus Obermayer, editors,
  \emph{Advances in Neural Information Processing Systems ({NIPS})}, pages
  1547--1554. {MIT} Press, 2002.

\bibitem[Poupart and Boutilier(2013)]{poupart2013value}
Pascal Poupart and Craig Boutilier.
\newblock Value-directed belief state approximation for {POMDPs}.
\newblock \emph{CoRR}, abs/1301.3887, 2013.
\newblock URL \url{http://arxiv.org/abs/1301.3887}.

% \bibitem[Puterman(1994)]{puterman94markov}
% Martin~L. Puterman.
% \newblock \emph{Markov Decision Processes---Discrete Stochastic Dynamic
%   Programming}.
% \newblock John Wiley \& Sons, Inc., 1994.
% 
\bibitem[Ravindran and Barto(2004)]{ravindran2004approximate}
Balaraman Ravindran and Andrew~G. Barto.
\newblock Approximate homomorphisms: A framework for non-exact minimization in
  {M}arkov {D}ecision {P}rocesses, 2004.
% 
% \bibitem[Russell and Norvig(2003)]{russel2003artificial}
% Stuart~J. Russell and Peter Norvig.
% \newblock \emph{Artificial Intelligence: A Modern Approach}.
% \newblock Pearson Education, 3 edition, 2003.
% 
% \bibitem[Schrittwieser et~al.(2019)Schrittwieser, Antonoglou, Hubert, Simonyan,
%   Sifre, Schmitt, Guez, Lockhart, Hassabis, Graepel,
%   et~al.]{schrittwieser2019mastering}
% Julian Schrittwieser, Ioannis Antonoglou, Thomas Hubert, Karen Simonyan,
%   Laurent Sifre, Simon Schmitt, Arthur Guez, Edward Lockhart, Demis Hassabis,
%   Thore Graepel, et~al.
% \newblock Mastering atari, go, chess and shogi by planning with a learned
%   model.
% \newblock \emph{arXiv preprint arXiv:1911.08265}, 2019.
% 
% \bibitem[Silver et~al.(2017)Silver, van Hasselt, Hessel, Schaul, Guez, Harley,
%   Dulac-Arnold, Reichert, Rabinowitz, Barreto, et~al.]{silver2017predictron}
% David Silver, Hado van Hasselt, Matteo Hessel, Tom Schaul, Arthur Guez, Tim
%   Harley, Gabriel Dulac-Arnold, David Reichert, Neil Rabinowitz, Andre Barreto,
%   et~al.
% \newblock The predictron: End-to-end learning and planning.
% \newblock In \emph{Proceedings of the 34th International Conference on Machine
%   Learning-Volume 70}, pages 3191--3199. JMLR. org, 2017.
% 
% \bibitem[Sutton(1988)]{sutton88learning}
% Richard~S. Sutton.
% \newblock Learning to predict by the methods of temporal differences.
% \newblock \emph{Machine Learning}, 3:\penalty0 9--44, 1988.
% 
\bibitem[Sutton(1995)]{sutton1995tdmodels}
Richard~S. Sutton.
\newblock {TD} models: Modeling the world at a mixture of time scales.
\newblock In \emph{Proceedings of the Twelfth International Conference on
  Machine Learning}, pages 531--539, 1995.
% 
% \bibitem[Sutton and Barto(2018)]{sutton2018reinforcement}
% Richard~S. Sutton and Andrew~G. Barto.
% \newblock \emph{Reinforcement Learning: An Introduction}.
% \newblock MIT Press, 2018.
% \newblock URL
%   \url{https://mitpress.mit.edu/books/reinforcement-learning-second-edition}.
% \newblock 2nd edition.
% 
% \bibitem[Sutton et~al.(1999)Sutton, Precup, and Singh]{sutton1999between}
% Richard~S Sutton, Doina Precup, and Satinder Singh.
% \newblock Between mdps and semi-mdps: A framework for temporal abstraction in
%   reinforcement learning.
% \newblock \emph{Artificial intelligence}, 112\penalty0 (1-2):\penalty0
%   181--211, 1999.
% 
% \bibitem[Sutton et~al.(2008)Sutton, Szepesv\'{a}ri, Geramifard, and
%   Bowling]{sutton2008dyna}
% Richard~S. Sutton, Csaba Szepesv\'{a}ri, Alborz Geramifard, and Michael
%   Bowling.
% \newblock Dyna-style planning with linear function approximation and
%   prioritized sweeping.
% \newblock In \emph{Proceedings of the Conference on Uncertainty in Artificial
%   Intelligence ({UAI})}, page 528–536, 2008.
% 
% \bibitem[Szepesv{\'a}ri(2010)]{szepesvari2010algorithms}
% Csaba Szepesv{\'a}ri.
% \newblock \emph{Algorithms for Reinforcement Learning}.
% \newblock Synthesis Lectures on Artificial Intelligence and Machine Learning.
%   Morgan {\&} Claypool Publishers, 2010.
% 
% \bibitem[Tamar et~al.(2016)Tamar, Wu, Thomas, Levine, and
%   Abbeel]{tamar2016value}
% Aviv Tamar, Yi~Wu, Garrett Thomas, Sergey Levine, and Pieter Abbeel.
% \newblock Value iteration networks.
% \newblock In \emph{Advances in Neural Information Processing Systems}, pages
%   2154--2162, 2016.

\end{thebibliography}


==> related_work_backup.tex <==

In this section we briefly discuss how variants of the value equivalence principle might be applied (with a slight abuse of notation) to a richer set of Bellman operators $\mathcal{T}v$, and use this taxonomy to provide insight into prior work. 
%
First, value equivalence can be applied to an uncontrolled Markov reward process; the resulting operator $\mathcal{T}$ is analogous to having a single policy in $\Pi$. Second, it can be applied over $n$ steps, using a Bellman operator $\Tpi^n$ that rolls the model forward $n$ steps: $\Tpi^n [v](s) = \E_{\pi}[R_{t+1} + ... + \gamma^{n-1} R_{t+n} + \gamma^n v_{\pi}(S_{t+n}) | S_t = s]$, or a $\lambda$-weighted average $\Tpi^\lambda$~\cp{bertsekas96neuro-dynamic}. Third, it can be applied to the Bellman optimality operator, $\mathcal{T}_{G_v} [v](s) = \max_a \E[R + \gamma v(S’) | s, a] $, where $G_v$ is the ``greedy'' policy induced by $v$ defined as $G_v(a|s) = \ind\{a = \argmax_{a'} \mathbb{E}[R + \gamma v(S’) | s, a']\}$. This idea can also be extended to an $n$-step greedy search operator, $\mathcal{T}_{G_v^n} [v](s) = \max_{a_1, ..., a_n} \mathbb{E}[R_{t+1} + ... + \gamma^{n-1} R_{t+n} + \gamma^n v(S_{t+n}) | S_t = s, A_{t} = a_1, ..., A_{t+n} = a_n]$. Finally, it can be applied to a non-stationary sequence of functions, $\mathcal{T} v_t = \mathcal{T}^* v_t$, such as successive estimates of the value function, where $\mathcal{T}^*$ is an appropriate Bellman operator applied to the true model $m^*$ (see Appendix \ref{sec:lit_review}).

The following table suggests connections to related methods used in prior work. For each method, we instantiate a value equivalence principle with a Bellman operator $\mathcal{T}$, policies $\Pi$, and functions $\mathcal{V}$, and conjecture that this captures the essential idea underlying each method for model-learning, acknowledging that we ignore many important details. 
Only MuZero includes both many policies and many functions, which may be sufficient to approximately span the policy and function space required to plan in complex environments; this perhaps explains its stronger empirical performance. 

\begin{tabular}{llll}
\label{tab:related}
Algorithm & VE Principle & Policies $\Pi$ & Functions $\mathcal{V}$ \\
\hline 
Predictron \cite{silver2017predictron} & $\mathcal{T}^\lambda v_t = \mathcal{T}^* v_t$ & None & Value functions for pseudo-rewards \\
VIN \cite{tamar2016value} & $\mathcal{T}_{G_{v_t}}^n v_t = \mathcal{T}^* v_t$ & $G_{v_t}$ & Value function \\
TreeQN \cite{farquhar2018treeqn} & $\mathcal{T}_{G_{v_t}^n}^n v_t = \mathcal{T}^* v_t$ & $G_{v_t}^n$ & Value function \\
VPN \cite{oh2017value} & $\mathcal{T}_{\pi_t}^n v_t = \mathcal{T}^* v_t$ & $\{a_1, ..., a_n\}$ & Value function \\
MuZero \cite{schrittwieser2019mastering} & $\mathcal{T}_{\pi_t}^n v_t = \mathcal{T}^* v_t$ & $\{a_1, ..., a_n\}$ & Distributional value, policy targets from search \\
\end{tabular}

==> related_work_bk.tex <==

% discuss Joseph et al. [2013]
%Kavosh Asadi, Evan Cater, Dipendra Misra, and Michael L. Littman. Equivalence between wasserstein
% and value-aware model-based reinforcement learning. In FAIM Workshop on Prediction and
% Generative Modeling in Reinforcement Learning, 2018. 3

In this paper we argue that models should be learned deliberately taking into account the underlying the RL problem. This notion has been explored befre in the literature. \ca{farahmand2013value}'s \cp{farahmand2013value,farahmand2017value} \emph{Value-Aware Model Learning} (VAML) is based on a premise similar to ours. They study a variant of~(\ref{eq:ve_loss}) that considers the worst-case choice of $v \in \V$; based on this formulation, they provide an expression for the gradient when the value-function approximation \vt\ is linear and the model \pt\ belongs to the exponential family. Later, \ct{farahmand2018iterative} also considered the case in which the model is learned iteratively as the agent interacts with the environment. Both versions of VAML come with finite sample-error guarantees~\cp{farahmand2013value,farahmand2017value,farahmand2018iterative}. 

Recently, there have been several works of a more empirical nature that can be understood as applications of the value-equivalence principle, like \ctp{silver2017predictron} \emph{Predictron}, \ctp{oh2017value} \emph{Value-Prediction Networks}, \ctp{farquhar2018treeqn} \emph{TreeQN}, and \ctp{schrittwieser2019mastering} \emph{MuZero}. Although these works vary considerably in the details, they all build on the idea of learning an abstract model that ignores irrelevant aspects of the environment and focuses instead on the features that are crucial for the solution of an RL problem. Roughly speaking, this is accomplished by ensuring that sequences of actions lead to the same sum of rewards in the model and environment. This can be interpreted as a generalizaton of the concept of value equivalence, given in Definition~\ref{def:ve}, from a single to multiple applications of the Bellman operator---an observation corroborated by the fact that the losses minimized by these methods closely resemble the empirical value-equivalence loss in~(\ref{eq:ve_loss_emp}). 


We consider the work on VAML complementary to ours: while we focus on the characterization of the space of value-equivalent models, they focus on the solution and analysis of the induced optimization problem.
The connection between the value-equivalence principle and the works above is beneficial to both: if one hand the current investigation provides a theoretical justification for some of the experiments successfully carried out in the past, on the other hand these experiments also provide additional empirical validation for the arguments put forward in this paper.   

